Convergence Analysis of MAP based Blur Kernel Estimation

One popular approach for blind deconvolution is to formulate a maximum a posteriori (MAP) problem with sparsity priors on the gradients of the latent image, and then alternatingly estimate the blur kernel and the latent image. While several successful MAP based methods have been proposed, there has been much controversy and confusion about their convergence, because sparsity priors have been shown to prefer blurry images to sharp natural images. In this paper, we revisit this problem and provide an analysis on the convergence of MAP based approaches. We first introduce a slight modification to a conventional joint energy function for blind deconvolution. The reformulated energy function yields the same alternating estimation process, but more clearly reveals how blind deconvolution works. We then show the energy function can actually favor the right solution instead of the no-blur solution under certain conditions, which explains the success of previous MAP based approaches. The reformulated energy function and our conditions for the convergence also provide a way to compare the qualities of different blur kernels, and we demonstrate its applicability to automatic blur kernel size selection, blur kernel estimation using light streaks, and defocus estimation.

==> algorithm.tex <==
\section{Decomposition of $S$ and $R$}
\label{sec:decomposition_S_R}

After obtaining $B$, we decompose it into $S$ and $R$ by optimizing an energy function.
To simplify formulation and optimization of an energy function, we take logarithm to our model as done in \cite{} and get $i(p) = \log I(p) = b(p) + t(p) = r(p) + s(p) + t(p)$ where $b(p) = \log B(p)$, $t(p) = \log T(p)$, $s(p) = \log S(p)$ and $r(p) = \log R(p)$.
Using the variables in the logarithmic domain, we minimize the following energy function:
\begin{equation}
f(s, r) = f^r(r) + f^s(s) + f^{sn}(s)
\label{eq:energy_function}
\end{equation}
subject to $b(p) = s(p) + r(p)$. In \Eq{energy_function}, $f^r(r)$ is a piecewise constant constraint on $r$, $f^s(s)$ is a piecewise smooth constraint on $s$, and $f^{sn}(s)$ is a surface normal based constraint on $s$.
In the following, we will describe each constraint in more detail.

\subsection{Surface Normal based Shading Constraint $f^{sn}(s)$}
\textbf{Locally linear embedding manifold preserving constraint} \\
For lambertian surface, shading $S$ can be calculated by taking the dot product of the lighting direction
vector $L$ and surface normal vector $N$:
\begin{equation}
S(p) = L\cdot N(p).
\end{equation}
In a local window, lighting condition of neighbor pixels can be considered that they are the same.

If a surface normal of pixel $p$ is expressed as a linear combination of those of neighbor pixels $q \in \mathcal{N}_{nl}(p)$, i.e. $N(p) = \sum_{q \in \mathcal{N}_{nl}(p)} w_{pq}^{N}N(q)$ where $w_{pq}^{N}$ is linear combination weights, then a shading of the pixel $p$ also can be expressed as a linear combination of same neighbors' shading using same weights $w_{pq}^{N}$:
\begin{equation}
S(p) = L \cdot \sum_{q \in \mathcal{N}_{nl}(p)} w_{pq}^{N}N(q) = \sum_{q \in \mathcal{N}_{nl}(p)} w_{pq}^{N}L \cdot N(q) = \sum_{q \in \mathcal{N}_{nl}(p)} w_{pq}^{N}S(q)
\label{eq:lle}
\end{equation}
To estimate the linear combination weights $w_{pq}^{N}$, we follows the work of Chen et al., which uses Locally Linear Embedding (LLE) to represent the manifold structure of an image and edits the image with manifold preserving constraint. LLE projects a data from high dimension to low dimension by representing a point as a linear combination of its neighbors in the feature space. For surface normal $N(p)$, we calculate linear combination weights $w_{pq}^N$ by minimizing following energy function:
\begin{equation}
\sum_{p \in P} \| N(p) - \sum_{q \in \mathcal{N}_{nl}(p)} w_{pq}^{N}N(q) \|^2,
\end{equation}
subject to $\sum_{q \in \mathcal{N}_{nl}(p)} w_{pq}^{N} = 1$, and $P$ is a set of every pixel.
$\mathcal{N}_{nl}(p)$ is a set of $k$-nearest neighbor pixels of pixel $p$.
To find local neighbor pixels, we estimate Euclidean distance between two pixels using feature vector $(x(p), y(p), z(p), nx(p), ny(p), nz(p))$ and find $k$-nearest neighbors, where $x(p), y(p), z(p)$ are the location of pixel $p$ in three-dimensional space and $nx(p), ny(p), nz(p)$ are the surface normal direction of pixel $p$.

From equation (\ref{eq:lle}), we enforce that the manifold structure of the shading follows the same manifold structure of surface normal by minimizing the following energy function:
\begin{equation}
F^{LLE}(S) = \sum_{p \in P}\left(S(p) - \sum_{q \in \mathcal{N}_{LLE}(p)} w_{pq}^{LLE}S(q)\right)^2.
\end{equation}

\begin{figure}[t]
\centering
\begin{tabular}{ccc}
\includegraphics[scale=0.18]{dummy} & \includegraphics[scale=0.18]{dummy}  & \includegraphics[scale=0.18]{dummy}
\end{tabular} 
\caption{\textbf{(Dummy)} Effects of local and non-local LLE constraints, Left: input image, Top Center and Top Right: results only using local LLE constraint, Bottom Center and Bottom Right: results using local and non-local LLE constraint }
\label{fig:locallle}
\end{figure}

In the input image of Fig.~\ref{fig:locallle}., we expect that XX and XX have similar shading corresponds to their similar surface normal.
We call this property as \textit{global shading consistency}.
To enforce \textit{global shading consistency}, we introduce non-local LLE constraint what formulate similarity among the distant pixels. Similar to the local LLE constraint, we use LLE manifold estimation, but instead of using feature vector $(x(p), y(p), z(p), nx(p), ny(p), nz(p))$ to represent the pixel, we only use $(nx(p), ny(p), nz(p))$ to find k-nearest neighbor pixels regardless of their location. This constraint is formulated as minimizing following energy function
\begin{equation}
F^{GSC}(S_B) = \sum_{p \in P}\left(S_B(p) - \sum_{q \in \mathcal{N}_{GSC}(p)} w_{pq}^{GSC}S_B(q)\right)^2
\end{equation}
By adding the constraint to our optimization framework, we get the shading which shows more globally consistent shading than without adding it (Fig.~\ref{fig:locallle} Bottom).
 \\
\textbf{Sub-sampling the manifold structure} \\
Even if LLE manifold preserving constraint is very powerful, applying it to the real input scene is difficult.
Raw depth image from the Microsoft Kinect is noisy due to the limitation of the device
and surface normal map made from the raw depth image is also noisy, especially for the edges.
For this reason, constraint with manifold structure captured by every pixel of the
image is unstable, and causes noisy shading result.

To solve this problem, we used a sub-sampling based propagation strategy inspired by Boyadzhiev's work [?].
Our method enforce the manifold structure of the shading image using only reliable anchor pixels.
Because complex scene geometry causes severe depth noise, we would better to choose anchor pixels in smooth area.
If the surface normal varies rapidly in a local window, this window may include edge or other complex geometry.
In this perspective, we estimated the variance of overlapping patches around each pixel as a surface smoothness measurement.
We divided an image into uniform grids and chose a pixel whose variance is the lowest as anchor pixel in each grid.

After applying sub-sampling, the manifold preserving constraint can be updated as:
\begin{equation}
\begin{split}
F^{LLE'}(S_B) = \sum_{p \in P_A}\left(S_B(p) - \sum_{q \in \mathcal{N'}_{LLE}(p)} w_{pq}^{N}S_B(q)\right)^2 \\
F^{GSC'}(S_B) = \sum_{p \in P_A}\left(S_B(p) - \sum_{q \in \mathcal{N'}_{GSC}(p)} w_{pq}^{GSC}S_B(q)\right)^2
\end{split}
\end{equation}
where $P_A$ is the set of anchor pixels, and $\mathcal{N'}_{LLE}(p)$, $\mathcal{N'}_{GSC}$ are the sets of $k$-nearest neighbor pixels found in $P_A$ using their distance measures. \\ \\

\subsection{Shading Constraint $f^s(s)$}
\textbf{Local shading propagation constraint} \\
Since we sub-sample the anchor pixels sparsely in the image,
most pixel pairs do not have any shading constraint between them.
Moreover, for adjacent pixels near to the edges whose chromaticity rapidly vary,
even there is no reflectance constraint between them.
For those pixels, it is impossible to solve the ambiguity between shading and reflectance.
Therefore, we need to propagate sub-sampled manifold structure through the whole image.
For propagation we use two local smoothness constraints for the shading.

As described in section 3.1, because we extract the textures from the image, small derivatives from reflectance
are removed. Therefore, in a local window $\omega_k$ whose reflectance is constant, 
we can assume that the local image structure of $B$ follows the same structure of shading $S$.
We exploit this assumption using a local shading constraint.

\textbf{이 아래, matting Laplacian을 쓰는 타당성에 대한 설명이 보충되어야 함. haze removal의 transmission map refinement에 inspired 되었다고 하는건 너무 막연한 것 같기도 함, guided filtering, 혹은 cross bilateral filtering과 비슷한 느낌이지만 energy minimization이라 엮어서 설명하기가 쉽지 않음.}
For the pixel similarity measure, we use matting Laplacian similarity on $B$.
We minimize the following cost function to guide the piecewise local smoothness of shading:
\begin{equation}
F^{IL}(S_B) = \sum_{k}^{K}\sum_{(i, j) \in \omega_k} w_{ij}^{SL} (S_B(i) - S_B(j))^2
\end{equation}
where $w_k$ is $k$-th local window, $w_{ij}^{SL}$ is matting Laplacian element, which is computed as:
\begin{equation}
w_{ij}^{SL} = \sum_{k | (i, j) \in \omega_k} \left( \delta_{ij} - \frac{1}{|\omega_k|} ( 1 + \left( B(i) - \mu^B_k \right) \\
  (\Sigma^B_k + \frac{\epsilon}{|\omega_k|} I_3)^{-1} \left( B(j) - \mu^B_k \right)  ) \right),
\end{equation}
where $\epsilon$ is regularizing parameter, $|\omega_k|$ is the number of pixels in the windows $\omega_k$,
$B_i$ and $B_j$ is the base image $B$ at pixels $i$ and $j$,
$\delta_{ij}$ is Kronecker delta, $\mu^{B}_{k}$ and $\Sigma^{B}_{k}$ are mean vector and covariance matrix of
$B$ in a window $\omega_k$, and $I_3$ is $3\times3$ identity matrix.

This constraint is a key advantage of removing the texture from the image. In the original image, image-based pixel similarity could not give any meaningful information about the shading because of the rich textures. In contrast, by removing texture from the image, we can approximate the structure of the shading image using the structure of the base image.

Second local smoothness constraint is based on surface normal. Even if the surface normal is noisy, it shows meaningful geometry information for smooth surface. By inspired [steve's] work, we formulate an energy function that enforces the local smoothness using surface normal difference between adjacent pixels. They uses binary threshold to determine whether adjacent pixels to be smooth or not. Instead of using binary threshold, we use continuous weighting function similar to the reflectance constraint we presented. Then we formulate the smoothness constraint as follow:
\begin{equation}
F^{SL}(S_B) = \sum_{p \in P}\sum_{q \in \mathcal{N}_{l}(p)} w^{SL}_{pq}\left(S_B(p) - S_B(q)\right)^2,
\end{equation}
where $w^{SL}_{pq} = \exp\left(-\frac{<N(p), N(q)>^2}{\sigma_n^2}\right)$.

Using these local propagation constraints, we can propagate the shading values according to
the local image structures and surface normal around the anchor points.
Fig.~\ref{fig:localshading} shows the effect of the local propagation constraint. Applying the local propagation constraint
gives clean shading near to the edges like middle of bookshelves.
In contrast, using only the sub-sampled non-local constraint with the local propagation constraint,
shading values near to the edges were unstable.
\begin{figure}[t]
\centering
\begin{tabular}{ccc}
\includegraphics[scale=0.18]{dummy} & \includegraphics[scale=0.18]{ContRefLLEReflectance}  & \includegraphics[scale=0.18]{ContRefLLEShading}\\ 
\includegraphics[scale=0.18]{dummy} & \includegraphics[scale=0.18]{FullAlgorithmReflectance}  & \includegraphics[scale=0.18]{FullAlgorithmShading}\\ 
\end{tabular} 
\caption{Results of applying the local propagation constraint, Top left: original image, Top center \& right: reflectance \& shading image without applying local constraints, Bottom center \& right: reflectance \& shading image with applying local constraints}
\label{fig:localshading}
\end{figure}

\subsection{Reflectance Constraint $f^r(r)$}
The constraint $f^r(r)$ is based on a simple assumption, which is used by many Retinex-based approaches~\cite{}:
if two neighboring pixels have the same chromaticity, their reflectance should be the same as well.
Based on this assumption, previous methods use a constraint defined as:
\begin{equation}
f^r(r) = \sum_{p\in P}\sum_{q\in \mathcal{N}_l(p)} w^r_b(p,q)\left(r(p)-r(q)\right)^2
\end{equation}
where $P$ is a set of every pixel and $\mathcal{N}_{l}(p)$ is a set of 8-adjacent pixels of $p$.
The weighting function $w^r_b(p,q)$ is a positive constant if the difference between the chromaticity at $p$ and $q$ is smaller than a certain threshold, and zero otherwise.
While this constraint looks fairly simple, it is critical to use a good threshold. However, finding a good threshold can be either time consuming~\cite{} or a heuristic job.

Instead of using a threshold, we use a weighting function $w^r_s(p,q)$, which is based on chromaticity difference between two pixels $p$ and $q$, and , which involves chromaticity difference in the form of angular distance between two directional vectors:
\begin{equation}
w^r_s(p,q) = \exp\left(-\frac{\left<C(p), C(q)\right>^2}{\sigma_c^2}\right) \left\{1 + \exp\left(-\frac{B(p)^2+B(q)^2}{\sigma_i^2}\right) \right\},
\label{eq:continuous}
\end{equation}
where $C(p) = B(p)/|B(p)|$ is a normalized 3D vector consisting of RGB color channels, and $\left<C(p), C(q)\right>$ is the inner product of $C(p)$ and $C(q)$.
The first exponential term measures similarity between the chromaticity $C(p)$ and $C(q)$ using their angular distance.
The first term becomes $1$ if $C(p) = C(q)$ and becomes close to $0$ if $C(p)$ and $C(q)$ are different from each other, so that consistency between neighboring pixels can be promoted only when $C(p)$ and $C(q)$ are close to each other.
The second exponential term is a darkness weight.
Due to the nature of imaging sensors, dark pixels suffer from noise more than bright pixels, causing severe chromaticity noise in dark regions such as shadow~(\Fig{chromanoise}).
Thus, the second term gives larger weights to dark pixels to overcome such chromaticity noise.
Using the weighting function $w^r_s(p,q)$, our constraint $f^r(r)$ is defined as:
\begin{equation}
f^r(r) = \sum_{p\in P}\sum_{q\in \mathcal{N}_l(p)} w^r_s(p,q)\left(r(p)-r(q)\right)^2 .
\end{equation}

\begin{figure}[t]
\centering
\begin{tabular}{ccc}
\includegraphics[width=5cm]{chromanoiseinput} & \includegraphics[width=5cm]{chromanoise} & \includegraphics[width=1.88cm]{chromanoisemag}
\end{tabular} 
\caption{Difference in chromaticity noise  between brighter region (black box) and darker region(green box), Left: input image, Center: chromaticity image, Right: magnified views of regions}
\label{fig:chromanoise}
\end{figure}

\subsection{Optimization}

%\sunghyun{=====================}
%
%In this paper, we propose a new image model which explicitly involves
%the texture in it. An image $I$ can be considered as the product of base layer $B$ and texture layer $T$.
%By representing the base layer $B$ as the product of the base reflectance $R_B$ and the base shading $S_B$,
%intrinsic image decomposition process is rewritten as:
%\begin{equation}
%I(p) = S(p)R(p) = B(p)T(p) = R_B(p)S_B(p)T(p).
%\end{equation}
%By extracting the texture from an image, two assumptions on $R_B$ and $S_B$ hold.
%\begin{itemize}
%	\item $R_B$ is piecewise constant. Because we extract the texture from $R$, only large image derivatives come from reflectance remain in $B$.
%	\item In a local window whose reflectance is constant, the image structure of $S_B$ follows that of $B$. Because only large image derivatives from reflectance remains in $B$, we can consider small image derivatives as shading changes.
%\end{itemize}
%
%In following sections, we propose a intrinsic image decomposition algorithm using structure-texture separation.
%Our algorithm consists of two-step. First we use an structure-texture separation
%algorithm to get base image $B$ which properly fits our image model. Then we decompose base image $B$ into
%shading image $S_B$ and reflectance image $R_B$ using a variational method.
%To disambiguate the ill-posedness of decomposition, we propose one reflectance constraint and two shading constraints
%complementary to each other on above assumptions.
%
%\subsection{Structure-texture Separation}
%In this step, we use an image filtering method to extract the base image $B$ from the input image $I$.
%Based on our new image model, $B$ is the product of base shading $S_B$ and base reflectance $R_B$.
%Thus, we need to use structure-texture separation method which well preserves shading information
%in base image $B$ during the separation.
%
%Recent variational methods [L0, RTV] for structure-texture separation
%do not fit to our purpose since they suppresses the small image gradient, which comes from the shading during the separation.
%In contrast, filtering-based method [regcovsmooth] which uses the image intensity as an texture descriptor element
%preserves shading well during the separation, so we use this method to get base image $B$.
%Using author's Matlab implementation which is publicly available in the web,
%we extract the base image $B$ from the input RGB image.
%Fig.~\ref{fig:structure} shows that the separation method successfully removes the textures on the cushion
%and the floor while preserving the shading on the sofa.
%\begin{figure}[t]
%\centering
%\begin{tabular}{ccc}
%\includegraphics[scale=0.18]{input} & \includegraphics[scale=0.18]{structure}  & \includegraphics[scale=0.18]{texture}\\ 
%(a) Input & (b) Structure Layer & (c) Texture Layer\\
%\end{tabular} 
%\caption{Results of shading-preserving structure-texture separation}
%\label{fig:structure}
%\end{figure}
%
%\subsection{Reflectance Constraint}
%Our reflectance constraint is based on the simple assumption what Retinex-based approaches[?][?][?] assume:
%if two neighboring pixels have the same chromaticity, reflectance of those are also the same.
%Nevertheless, finding proper threshold to classify pixels who have the same chromaticity is
%time consuming [steve texture], or a heuristic job.
%
%Instead of using binary decision to choose whether adjacent pixels have the same reflectance or not,
%we use weighting function $w_{pq}$ which involves chromaticity differences in form of angular distance between directional vectors:
%\begin{equation}
%\omega^R_{pq} = \exp\left(-\frac{<C(p), C(q)>^2}{\sigma_c^2}\right) * \left(1 + \exp\left(-\frac{I(p)^2+I(q)^2}{\sigma_i^2}\right) \right),
%\label{eq:continuous}
%\end{equation}
%where $C(p) = I(p)/|I(p)|$, and $<A, B> = A \cdot B$.
%
%In equation (\ref{eq:continuous}), first exponential term is chromaticity similarity of two adjacent pixels $p$ and $q$.
%Since chromaticity is directional vector, we used angular distance rather than Euclidean distance.
%Second exponential term is darkness weight. In commercial RGB-D sensor, darker pixels suffer from a lot of noise
%than brighter pixels. It introduce chromaticity noise in dark regions such as shadow (Fig.~\ref{fig:chromanoise}).
%Because of this chromaticity noise issue, weighting function without considering the pixel intensity
%can enforce dissimilarity between pixels who should have the same reflectance.
%To handle this chromaticity noise, we give more similarity between darker pixels than brighter pixels.
%
%Using this similarity function we introduce following energy function which enforces smoothness between adjacent pixels when it is minimized:
%\begin{equation}
%F^{R}(R) = \sum_{p \in P}\sum_{q \in \mathcal{N}_{l}(p)} w^R_{pq}\left(R(p) - R(q)\right)^2,
%\end{equation}
%where $P$ is a set of every pixel and $\mathcal{N}_{l}(p)$ is a set of 8-adjacent pixels of $p$.
%
%\begin{figure}[t]
%\centering
%\begin{tabular}{ccc}
%\includegraphics[width=5cm]{chromanoiseinput} & \includegraphics[width=5cm]{chromanoise} & \includegraphics[width=1.88cm]{chromanoisemag}
%\end{tabular} 
%\caption{Difference in chromaticity noise  between brighter region (black box) and darker region(green box), Left: input image, Center: chromaticity image, Right: magnified views of regions}
%\label{fig:chromanoise}
%\end{figure}
%
%\subsection{Shading Constraints}
%\textbf{Locally linear embedding manifold preserving constraint} \\
%For lambertian surface, shading $S$ can be calculated by taking the dot product of the lighting direction
%vector $L$ and surface normal vector $N$:
%\begin{equation}
%S(p) = L\cdot N(p).
%\end{equation}
%In a local window, lighting condition of neighbor pixels can be considered that they are the same.
%
%If a surface normal of pixel $p$ is expressed as a linear combination of those of neighbor pixels $q \in \mathcal{N}_{nl}(p)$, i.e. $N(p) = \sum_{q \in \mathcal{N}_{nl}(p)} w_{pq}^{N}N(q)$ where $w_{pq}^{N}$ is linear combination weights, then a shading of the pixel $p$ also can be expressed as a linear combination of same neighbors' shading using same weights $w_{pq}^{N}$:
%\begin{equation}
%S(p) = L \cdot \sum_{q \in \mathcal{N}_{nl}(p)} w_{pq}^{N}N(q) = \sum_{q \in \mathcal{N}_{nl}(p)} w_{pq}^{N}L \cdot N(q) = \sum_{q \in \mathcal{N}_{nl}(p)} w_{pq}^{N}S(q)
%\label{eq:lle}
%\end{equation}
%To estimate the linear combination weights $w_{pq}^{N}$, we follows the work of Chen et al., which uses Locally Linear Embedding (LLE) to represent the manifold structure of an image and edits the image with manifold preserving constraint. LLE projects a data from high dimension to low dimension by representing a point as a linear combination of its neighbors in the feature space. For surface normal $N(p)$, we calculate linear combination weights $w_{pq}^N$ by minimizing following energy function:
%\begin{equation}
%\sum_{p \in P} \| N(p) - \sum_{q \in \mathcal{N}_{nl}(p)} w_{pq}^{N}N(q) \|^2,
%\end{equation}
%subject to $\sum_{q \in \mathcal{N}_{nl}(p)} w_{pq}^{N} = 1$, and $P$ is a set of every pixel.
%$\mathcal{N}_{nl}(p)$ is a set of $k$-nearest neighbor pixels of pixel $p$.
%To find local neighbor pixels, we estimate Euclidean distance between two pixels using feature vector $(x(p), y(p), z(p), nx(p), ny(p), nz(p))$ and find $k$-nearest neighbors, where $x(p), y(p), z(p)$ are the location of pixel $p$ in three-dimensional space and $nx(p), ny(p), nz(p)$ are the surface normal direction of pixel $p$.
%
%From equation (\ref{eq:lle}), we enforce that the manifold structure of the shading follows the same manifold structure of surface normal by minimizing the following energy function:
%\begin{equation}
%F^{LLE}(S) = \sum_{p \in P}\left(S(p) - \sum_{q \in \mathcal{N}_{LLE}(p)} w_{pq}^{LLE}S(q)\right)^2.
%\end{equation}
%
%\begin{figure}[t]
%\centering
%\begin{tabular}{ccc}
%\includegraphics[scale=0.18]{dummy} & \includegraphics[scale=0.18]{dummy}  & \includegraphics[scale=0.18]{dummy}
%\end{tabular} 
%\caption{\textbf{(Dummy)} Effects of local and non-local LLE constraints, Left: input image, Top Center and Top Right: results only using local LLE constraint, Bottom Center and Bottom Right: results using local and non-local LLE constraint }
%\label{fig:locallle}
%\end{figure}
%
%In the input image of Fig.~\ref{fig:locallle}., we expect that XX and XX have similar shading corresponds to their similar surface normal.
%We call this property as \textit{global shading consistency}.
%To enforce \textit{global shading consistency}, we introduce non-local LLE constraint what formulate similarity among the distant pixels. Similar to the local LLE constraint, we use LLE manifold estimation, but instead of using feature vector $(x(p), y(p), z(p), nx(p), ny(p), nz(p))$ to represent the pixel, we only use $(nx(p), ny(p), nz(p))$ to find k-nearest neighbor pixels regardless of their location. This constraint is formulated as minimizing following energy function
%\begin{equation}
%F^{GSC}(S_B) = \sum_{p \in P}\left(S_B(p) - \sum_{q \in \mathcal{N}_{GSC}(p)} w_{pq}^{GSC}S_B(q)\right)^2
%\end{equation}
%By adding the constraint to our optimization framework, we get the shading which shows more globally consistent shading than without adding it (Fig.~\ref{fig:locallle} Bottom).
% \\
%\textbf{Sub-sampling the manifold structure} \\
%Even if LLE manifold preserving constraint is very powerful, applying it to the real input scene is difficult.
%Raw depth image from the Microsoft Kinect is noisy due to the limitation of the device
%and surface normal map made from the raw depth image is also noisy, especially for the edges.
%For this reason, constraint with manifold structure captured by every pixel of the
%image is unstable, and causes noisy shading result.
%
%To solve this problem, we used a sub-sampling based propagation strategy inspired by Boyadzhiev's work [?].
%Our method enforce the manifold structure of the shading image using only reliable anchor pixels.
%Because complex scene geometry causes severe depth noise, we would better to choose anchor pixels in smooth area.
%If the surface normal varies rapidly in a local window, this window may include edge or other complex geometry.
%In this perspective, we estimated the variance of overlapping patches around each pixel as a surface smoothness measurement.
%We divided an image into uniform grids and chose a pixel whose variance is the lowest as anchor pixel in each grid.
%
%After applying sub-sampling, the manifold preserving constraint can be updated as:
%\begin{equation}
%\begin{split}
%F^{LLE'}(S_B) = \sum_{p \in P_A}\left(S_B(p) - \sum_{q \in \mathcal{N'}_{LLE}(p)} w_{pq}^{N}S_B(q)\right)^2 \\
%F^{GSC'}(S_B) = \sum_{p \in P_A}\left(S_B(p) - \sum_{q \in \mathcal{N'}_{GSC}(p)} w_{pq}^{GSC}S_B(q)\right)^2
%\end{split}
%\end{equation}
%where $P_A$ is the set of anchor pixels, and $\mathcal{N'}_{LLE}(p)$, $\mathcal{N'}_{GSC}$ are the sets of $k$-nearest neighbor pixels found in $P_A$ using their distance measures. \\ \\
%
%\textbf{Local shading propagation constraint} \\
%Since we sub-sample the anchor pixels sparsely in the image,
%most pixel pairs do not have any shading constraint between them.
%Moreover, for adjacent pixels near to the edges whose chromaticity rapidly vary,
%even there is no reflectance constraint between them.
%For those pixels, it is impossible to solve the ambiguity between shading and reflectance.
%Therefore, we need to propagate sub-sampled manifold structure through the whole image.
%For propagation we use two local smoothness constraints for the shading.
%
%As described in section 3.1, because we extract the textures from the image, small derivatives from reflectance
%are removed. Therefore, in a local window $\omega_k$ whose reflectance is constant, 
%we can assume that the local image structure of $B$ follows the same structure of shading $S$.
%We exploit this assumption using a local shading constraint.
%
%\textbf{이 아래, matting Laplacian을 쓰는 타당성에 대한 설명이 보충되어야 함. haze removal의 transmission map refinement에 inspired 되었다고 하는건 너무 막연한 것 같기도 함, guided filtering, 혹은 cross bilateral filtering과 비슷한 느낌이지만 energy minimization이라 엮어서 설명하기가 쉽지 않음.}
%For the pixel similarity measure, we use matting Laplacian similarity on $B$.
%We minimize the following cost function to guide the piecewise local smoothness of shading:
%\begin{equation}
%F^{IL}(S_B) = \sum_{k}^{K}\sum_{(i, j) \in \omega_k} w_{ij}^{SL} (S_B(i) - S_B(j))^2
%\end{equation}
%where $w_k$ is $k$-th local window, $w_{ij}^{SL}$ is matting Laplacian element, which is computed as:
%\begin{equation}
%w_{ij}^{SL} = \sum_{k | (i, j) \in \omega_k} \left( \delta_{ij} - \frac{1}{|\omega_k|} ( 1 + \left( B(i) - \mu^B_k \right) \\
%  (\Sigma^B_k + \frac{\epsilon}{|\omega_k|} I_3)^{-1} \left( B(j) - \mu^B_k \right)  ) \right),
%\end{equation}
%where $\epsilon$ is regularizing parameter, $|\omega_k|$ is the number of pixels in the windows $\omega_k$,
%$B_i$ and $B_j$ is the base image $B$ at pixels $i$ and $j$,
%$\delta_{ij}$ is Kronecker delta, $\mu^{B}_{k}$ and $\Sigma^{B}_{k}$ are mean vector and covariance matrix of
%$B$ in a window $\omega_k$, and $I_3$ is $3\times3$ identity matrix.
%
%This constraint is a key advantage of removing the texture from the image. In the original image, image-based pixel similarity could not give any meaningful information about the shading because of the rich textures. In contrast, by removing texture from the image, we can approximate the structure of the shading image using the structure of the base image.
%
%Second local smoothness constraint is based on surface normal. Even if the surface normal is noisy, it shows meaningful geometry information for smooth surface. By inspired [steve's] work, we formulate an energy function that enforces the local smoothness using surface normal difference between adjacent pixels. They uses binary threshold to determine whether adjacent pixels to be smooth or not. Instead of using binary threshold, we use continuous weighting function similar to the reflectance constraint we presented. Then we formulate the smoothness constraint as follow:
%\begin{equation}
%F^{SL}(S_B) = \sum_{p \in P}\sum_{q \in \mathcal{N}_{l}(p)} w^{SL}_{pq}\left(S_B(p) - S_B(q)\right)^2,
%\end{equation}
%where $w^{SL}_{pq} = \exp\left(-\frac{<N(p), N(q)>^2}{\sigma_n^2}\right)$.
%
%Using these local propagation constraints, we can propagate the shading values according to
%the local image structures and surface normal around the anchor points.
%Fig.~\ref{fig:localshading} shows the effect of the local propagation constraint. Applying the local propagation constraint
%gives clean shading near to the edges like middle of bookshelves.
%In contrast, using only the sub-sampled non-local constraint with the local propagation constraint,
%shading values near to the edges were unstable.
%\begin{figure}[t]
%\centering
%\begin{tabular}{ccc}
%\includegraphics[scale=0.18]{dummy} & \includegraphics[scale=0.18]{ContRefLLEReflectance}  & \includegraphics[scale=0.18]{ContRefLLEShading}\\ 
%\includegraphics[scale=0.18]{dummy} & \includegraphics[scale=0.18]{FullAlgorithmReflectance}  & \includegraphics[scale=0.18]{FullAlgorithmShading}\\ 
%\end{tabular} 
%\caption{Results of applying the local propagation constraint, Top left: original image, Top center \& right: reflectance \& shading image without applying local constraints, Bottom center \& right: reflectance \& shading image with applying local constraints}
%\label{fig:localshading}
%\end{figure}
%
%\subsection{Optimization}
%Incorporating every constraints described in previous sections, we minimize following energy function of shading $S_B$ and $R_B$:
%\begin{multline}
%F(S_B, R_B) = F^R(R) + F^{LLE'}(S_B) + F^{GSC'}(S_B) + F^{IL}(S_B) + F^{SL}(S_B),
%\end{multline}
%subject to $B(p) = S_B(p)R_B(p)$.
%
%To simplify the optimization, we took the logarithm to our model and got $b(p) = s_B(p) + r_B(p)$, where $b(p), s_B(p),$ and $r_B(p)$ are logarithm of base image, base reflectance, base shading respectively.
%We empirically found that proposed constraints also could represent the similarity between pixels in the logarithm domain, even for the LLE constraint. Then we rewrite the energy function:
%\begin{multline}
%F(s_B, s_B) = F^R(r_B) + F^{LLE'}(s_B) + F^{GSC'}(s_B) + F^{IL}(s_B) + F^{SL}(s_B).
%\label{eq:energy}
%\end{multline}
%Because $r_B(p) = b(p) - s_B(p)$, equation (\ref{eq:energy}) is a quadratic function of $s_B$, which can be expressed
%as large sparse linear system after some algebraic manipulations:
%\begin{equation}
%\bf{Cs_B = d},
%\end{equation}
%where $\bf{C, d}$ is constraints matrix and vector including  local and non-local constraints,
%and $\bf{s_B}$ is a vector concatenating every shading variables of image.
%Conjugate gradient method was used to solve the linear system.
